Detecting Gravitational Wave Anisotropies from Supermassive Black Hole Binaries

Several Pulsar Timing Array (PTA) collaborations have recently found evidence for a gravitational wave background (GWB) permeating our galaxy. The origin of this background is still unknown. Indeed, while the gravitational wave emission from inspiraling supermassive black hole binaries (SMBHB) is the primary candidate for its origin, several cosmological sources have also been proposed. One distinctive feature of SMBHB-generated backgrounds is the presence of GWB anisotropies stemming from the binaries distribution in the local Universe. However, none of the anisotropy searches performed to date reported a detection. In this work, we show that the lack of anisotropy detection is not currently in tension with a SMBHB origin of the background. We accomplish this by calculating the anisotropy detection probability of present and future PTAs. We find that a PTA with the noise characteristics of the NANOGrav 15-year data set had only a $~2\%-11\%$ probability of detecting SMBHB-generated anisotropies, depending on the properties of the SMBHB population. However, we estimate that for the IPTA DR3 data set these probabilities will increase to $~4\%-28\%$, putting more pressure on the SMBHB interpretation in case of a null detection. We also identify SMBHB populations that are more likely to produce detectable levels of anisotropies. This information could be used together with the spectral properties of the GWB to characterize the SMBHB population.

==> mock_data.tex <==
\subsection{Population Synthesis with \texttt{holodeck}}\label{subsec:smbhb_gen}
To generate SMBHB populations, we used the same procedure as in Ref.~\cite{ng+23_astro}, which we briefly summarize in this section. For more details, we refer the reader to Refs.~\cite{ng+23_astro, holodeck}.

\subsubsection{Galaxy Merger Rate}
As SMBHB are formed in galaxy mergers, one of the key ingredients needed to model SMBHB populations is the rate of such mergers. The comoving number density of galaxies mergers, $\eta_{\rm gal-gal}$, can be written as~\cite{Chen_2019}:
\begin{equation}\label{eq:galaxy merger rate}
    \frac{\partial^{3}\eta_\text{gal-gal}}{\partial m_{\star 1}\partial q_\star \partial z}=\frac{\Psi(m_{\star 1}z^\prime)}{m_{\star 1}\ln(10)}\frac{P(m_{\star 1},q_\star,z^\prime)}{T_\text{gal-gal}(m_{\star 1},q_\star,z^\prime)}\frac{\partial t}{\partial z^\prime},
\end{equation}
where $\Psi$ denotes the galaxy stellar-mass function (GSMF), $P$ the galaxy pair fraction and $T_\text{gal-gal}$ the galaxy merger time. Since the galaxy merger spans a finite timescale ($T_{\rm gal-gal}$), in Eq.~\eqref{eq:galaxy merger rate}, we distinguish between the redshift at which the galaxy pair form ($z' = z'[t]$ at some initial time $t$) and the redshift at which the system becomes a post-merger galaxy remnant ($z = z[t + T_{\rm gal-gal}]$).

The GSMF provides the differential number-density of galaxies per decade of stellar mass. Following Ref.~\cite{ng+23_astro}, we parametrize the GSMF as a single Schechter function~\cite{Schechter_1976}:
\begin{equation}
    \Psi(m_{\star1},z^{\prime}) = \ln(10)\Psi_{0}\cdot\bigg(\frac{m_{\star1}}{M_{\psi}}\bigg)^{\alpha_{\psi}}\exp\bigg(-\frac{m_{\star1}}{M_{\psi}}\bigg),
\end{equation}
where the phenomenological parameters $\Psi_0$, $M_\psi$ and $\alpha_\psi$ follow the redshift parametrization introduced in~\cite{Chen_2019}:
\begin{equation}
    \begin{split}
        \log_{10}(\Psi_0/\Mpc^{-3}) & = \psi_0 + \psi_z\cdot z\\
        \log_{10}(M_\psi/M_\odot) & = m_{\psi,0} + m_{\psi,z}\cdot z\\
        \alpha_\psi &= 1+\alpha_{\psi,0}+\alpha_{\psi,z}\cdot z
    \end{split}
\end{equation}
This parametrization introduces six free parameters for the GSMF. Of this six parameters, 
the mass normalization $\psi_0$ and the characteristic mass $m_{\psi,0}$ are allowed to vary in our analysis, while the remaining four are fixed to the fiducial values provided in Table~\ref{tab:fid_val}.

The galaxy pair fraction and merger time are kept fixed to fiducial power-law functions of the galaxy stellar mass, galaxy mass ratio, and initial redshift. For a full description of these functions we direct the reader to Ref.~\cite{ng+23_astro}.

\renewcommand{\arraystretch}{1.45}
\setlength{\tabcolsep}{0.3cm}
\begin{table}[t!]
    % \centering
    \begin{tabular}{ccc}
    \toprule
         {\bf Binary property} & {\bf Range} &  {\bf Number of bins} \\
        \hline
        $M/M_\odot$ & $[10^4,10^{12}]$   & 91 \\
        $q$ & $[10^{-3},1]$   & 81 \\
        $z$ & $[10^{-3},10]$   & 101 \\
        $f$ &    &  \\
    \bottomrule
    \end{tabular}
    \caption{Value ranges and number of logarithmically spaced bins for the SMBHB parameters.}
    \label{tab:binning}
\end{table}

\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{0.3cm}
\begin{table}[t!]
    % \centering
    \begin{tabular}{ccc}
    \toprule
         {\bf Model Component} & {\bf Parameter} &  {\bf Fiducial value} \\
        \hline
            \multirow{ 4}{*}{GSMF}    & $\psi_z$   & -0.60 \\
                    & $m_{\psi,z}$   & +0.11 \\
                    & $\alpha_{\psi,0}$   & -1.21 \\
                    & $\alpha_{\psi,z}$   & -0.03 \\

        \hline
         \multirow{2}{*}{$M_{\text{BH}}-M_\text{bulge}$} & $\alpha_\mu$     & 1.10 \\
                    & $f_{\star,\text{bulge}}$     & 0.615 \\
        \hline
         \multirow{3}{*}{$\dfrac{da}{dt}\bigg\vert_{\rm phenom}$}    & $a_c/{\rm pc}$  & $10^2$\\
                                        & $a_\text{init}/{\rm pc}$ & $10^4$\\
                                        & $\nu_\text{outer}$ & 2.5\\
    \bottomrule
    \end{tabular}
    \caption{Fiducial model parameters as presented in table B1 of Ref.~\cite{ng+23_astro}, based on Ref.~\cite{Chen_2019} for the GSMF, Refs.~\cite{Gültekin_2009, Kormendy_2013, McConnell_2013} for the $M_\text{BH}-M_\text{Bulge}$ relation and Refs.~\cite{Bluck_2014, Lang_2014} for the bulge fraction. The phenomenological hardening parameters are based on Refs~\cite{Kelley2017, ng+23_astro}. \AL{$a_{init}$ is 1e4 in our script and the ones i found for holodeck, but 1e3 in the holodeck paper}}
    \label{tab:fid_val}
\end{table}

\subsubsection{SMBH-Host Relation}
By populating galaxies with supermassive black holes (SMBHs), we can relate Eq.~\eqref{eq:galaxy merger rate} with the SMBHs merger rate. We populate the galaxies assuming a one-to-one correspondence between the host galaxy and the SMBH at its center. Specifically, we use assume that the SMBH mass, $M_{\rm BH}$, is related to the bulge mass of the host galaxy, $-M_{\rm bulge}$, according to the relation~\cite{}:
\begin{equation}
    \log_{10}(M_{\text{BH}}/M_{\odot})=\mu+\alpha_{\mu}\log_{10}\bigg(\frac{M_{\text{bulge}}}{10^{11}M_{\odot}}\bigg)+\mathcal{N}(0,\epsilon_\mu)\,
\end{equation}
where $\mathcal{N}(0,\epsilon_\mu)$ is a normally distributed random scatter with zero mean and standard deviation $\epsilon_\mu$; and $M_{\rm bulge}=f_{\star,{\rm bulge}}\cdot m_{\star}$ is the fraction of the galaxy stellar mass contained in the bulge. In our analysis, we vary the mass normalization $\mu$ and the scattering width $\epsilon_\mu$, while keeping the other parameters fixed to the fiducial values reported in Table~\ref{tab:fid_val}.

Using the $M_{\rm BH}-M_{\rm bulge}$ relation we can then translate the number density of galaxy mergers to the number density of SMBHB mergers:
\begin{equation}
    \frac{\partial^{3}\eta}{\partial M\partial q\partial z}=\frac{\partial^{3}\eta_\text{gal-gal}}{\partial m_{\star 1}\partial q_\star \partial z}\frac{\partial m_{\star 1}}{\partial M}\frac{\partial q_\star}{\partial q}\,.
\end{equation}

\subsubsection{Binary Evolution}
For binaries on circular orbits, the observer-frame GW frequency, $f$, is related to the binary's rest frame orbital frequency, $f_p$, as $f=2f_p/(1+z)$. The orbital frequency, in turn, is uniquely related to the binary orbital separation, $a$, according to $f_p^2=4\pi G M/a^3$.

The evolution of the binary system's orbital separation, $a$, is driven by a combination of GW emission and interactions with the astrophysical environment (i.e. stars and gas). The GW contribution to the binary hardening is given by~\cite{Peters_1964}:
\begin{equation}
    \frac{da}{dt}\bigg\vert_{\text{GW}}=-\frac{64G^3}{5c^5}\frac{m_1 m_2 M}{a^3}\,,
    \label{eq:hardening_gw}
\end{equation}
where $G$ is the gravitational constant. 
We describe environmental effects using a phenomenological model which aims to capture the overall effects of more complicated explicit binary evolution models, while introduing a small number of free parameters:
\begin{equation}
    \label{eq:hardening_pheno}
    \frac{da}{dt}\bigg\vert_{\text{phenom}}=H_{a}\bigg(\frac{a}{a_{c}}\bigg)^{1-\nu_\text{inner}}\bigg(1+\frac{a}{a_c}\bigg)^{\nu_\text{inner}-\nu_\text{outer}}.
\end{equation}
Here, two additional parameters $\nu_\text{inner}$ and $\nu_\text{outer}$ are introduced, dividing the hardening process into a small-separation and a large-separation regime with different power-law behaviours and a turnover at a critical separation $a_c$. While $\nu_\text{inner}$ is allowed to vary in our model, $\nu_\text{outer}$ is fixed to a standard literature value of $+2.5$~\cite{Kelley2017}. The total rate of binary evolution is obtained by summing the two contributions:
\begin{equation}
    \frac{da}{dt}= \frac{da}{dt}\bigg\vert_{\text{GW}} + \frac{da}{dt}\bigg\vert_{\text{phenom}}\,.
\end{equation}


The normalization of the phenomenological hardening rate, $H_{a}$, is determined by requiring that the binary lifetime, from the initial separation $a_{\rm initi}$ to the innermost stable circular orbit $a_{\rm isco}=6GM/c^2$, is given by a target $\tau_f$:
\begin{equation}\label{eq:hardening_time}
    \tau_{f}=\int_{a_\text{init}}^{a_\text{isco}}\bigg(\frac{da}{dt}\bigg)^{-1}da,
\end{equation}
The value of $\tau_f$ is a free parameter that we allow to vary in our analysis.

Given a model for the binary orbital evolution, we can write the number of SMBHB per given mass, mass-ratio, redshift, and log orbital frequency, as~\cite{}:
\begin{equation}\label{eq:num_den}
    \frac{\partial^4 N}{\partial M\partial q\partial z \partial \ln f_p} = \frac{\partial^{3}\eta}{\partial M\partial q \partial z}\cdot\tau(f_p)\cdot 4\pi c(1+z)d_c^2\,,
\end{equation}
where $d_c$ is the comoving distance of a source at redshift $z$, and $\tau(f_p)$ is the binary hardening timescale:
\begin{equation}
    \tau(f_p)\equiv f_p/(df_p/dt)= -\frac{2a}{3}\frac{da}{dt}\,.
\end{equation}

\subsubsection{Population Synthesis}
%For binaries on circular orbits, the sky and polarization-averaged GW emission is uniquely characterized by four quantities: the total \emph{binary mass} $M\equiv m_1+m_2$, where $m_1$ and $m_2$ are the masses of the SMBHs in the binary; the \emph{mass ratio} $q\equiv m_2/m_1\leq 1$; the \emph{binary's redshift} $z$; and the binary \emph{orbital frequency} $f_p$.

Given the continuous distribution for the number of binaries in Eq.~\eqref{eq:num_den}, we generate SMBHB populations by drawing the number of binaries in a given $(M,\,q,\,z,\,f_p)$ bin from a Poisson distribution centered around the expectation value
\begin{equation}
    N(M,q,z,f_p)=\frac{\partial^4 N}{\partial M\partial q\partial z \partial \ln f_p}\Delta M\, \Delta q\, \Delta z\, \Delta\ln f_p,
\end{equation}
where $(\Delta M,\,\Delta q,\,\Delta z,\,\Delta f_p)$ are the bin sizes for each SMBHB parameter. Details about the binning of the SMBHB parameter space are reported in Tab.~\ref{tab:binning}.

For each set of astrophysical parameters, $\{\psi_0,\,m_{\psi,0},\,\mu,\,\epsilon_\mu, \,\tau_f,\,\nu_{\rm inner}\}$, we generate 50 independent SMBHB populations. To ensure that the SMBHB populations considered in our analysis are consistent with the spectral properties of the observed GWB, the astrophysical parameters are randomly sampled from the posterior distributions derived in Ref.~\cite{ng+23_astro}.

\subsection{GWB Sky Maps}\label{subsec:sky_gen}
Given a mock SMBHB population, the next step consist in generating an associated GW sky, $\mathbf{P}$.
We start by assuming that each of the SMBHB is on a circular orbit, and assigning them the $M$, $q$, $z$, and $f_p$ values corresponding to their bin centers. We can then derive their sky and polarization-averaged strain as~\cite{Finn_2000}:
\begin{equation}\label{eq:binary_strain}
    h_s^{2}(f)=\frac{32}{5c^8}\frac{(G\mathcal{M})^{10/3}}{d_c^2}(2\pi f_p)^{4/3}\,,
\end{equation}
where $\mathcal{M}=M q^{3/5}/(1+q)^{6/5}$. This strain can then be translated into a characteristic strain using the power spectral density \cite{Rosado_2015}
\begin{equation}\label{eq:char_binary_strain}
    h_c^{2}(f)= f S_h(f)=h_s^{2}(f)\frac{f}{\Delta f}\,,
\end{equation}
where $\Delta f=1/T_\text{obs}$ denotes the GW frequency bin width. Due to the finite frequency resolution, the spectral density $S_h(f)$ is spread over $\Delta f$, which introduces a normalization factor $1/\Delta f$. 
\AM{explain where the $f/\Delta f$ is coming from.}
\AL{added something about this, but I'm not sure it's helping}
For each frequency bin, we then place the loudest 20 sources on random pixels of a sky-tesselation derived by using HEALpix~\cite{healpix}, and add their squared characteristic strain to the corresponding pixels. The remaining binaries are added to the sky map as an isotropic background (equally divided among all pixels) with a characteristic strain given by
\begin{equation}
    h^{2}_{c,\scriptscriptstyle{BG}}(f) = \sum_{M,q,z,f_p}N(M,q,z,f_p)h_c^2(f)\,,
\end{equation}
where the sum runs over all binaries expect the loudest 20.\footnote{To generate the mock sky maps we use $N_\text{side}=16$, resulting in a resolution of $12\cdot N_\text{side}^{2}=3072$ pixels. We have checked that the finite resolution effects on the induced pulsar-pair correlations are negligible for $N_\text{side}\geq16$. The anisotropy of the GWB is mainly captured by the loudest 10 sources in terms of spherical harmonic coefficients~\cite{gardiner2023background}, which we have confirmed also applies for our pixel basis.} The maps are then normalized such that $\int_{S^2}d\hat\Omega\,\mathbf{P}(\hat\Omega,f)=\sum_k P_{i,k}\Delta\hat\Omega_k=4\pi$.

To marginalize over the sky locations of the loudest sources, for each SMBHB population, we generate 30 independent sky maps per frequency bin. Given that we generate 50 SMBHB populations for each set of astrophysical parameters (see the previous section for details), we produce a total of 1500 sky maps per frequency bin for each set of astrophysical parameters. Examples of mock sky maps are provided in the upper panels of Fig.~\ref{fig:mock_sky}.

\begin{figure*}[htp!]
    \centering
    \includegraphics[width=\textwidth]{figs/map_examples.pdf}
    \caption{Examples for the GWB power distributions induced by SMBHB populations (upper panel) and the recovered $S/N$ sky maps from the analytical (middle panel) and numerical (lower panel) solution approach. The left panels illustrate the reconstruction of a SMBHB population with a statistically significant hot spot in the most sensitive region of the sky that is classified as detetcion of anisotropies in our analysis. The right panels show a SMBHB population that does not lead to a anisotropy detection.}
    \label{fig:mock_sky}
\end{figure*}

\subsection{Mock Correlations}\label{subsec:cor_gen}
The final step of the procedure consists in generating reconstructed cross-correlations for each of the mock GWB skies. For a given sky map, $P_{i,k}$, the expected cross-correlations are given by Eq.~\eqref{eq:theo_corr_disc}. However, realistic reconstructed correlations will substantially deviate from these expectation values due to the finite precision of our data. Therefore, we generate mock correlation values by sampling from a Gaussian distribution centered around the expected value given by Eq.~\eqref{eq:theo_corr_disc}, and with a standard deviation given by the cross-correlation uncertainties measured from the NANOGrav 15-year data set using the per-frequency (OS)~\cite{}.
 
% Maybe add in some information about optimal statistic
%Therefore, our ability to reconstruct anisotropies strongly depend on the frequency, with the second frequency bin at $f_\text{GW}\approx3.95$\nHz\ showing the best sensitivity.\\
%\begin{equation}
%    \sigma_{ab} = \bigg(\tr\bigg[\mathbf{N}_a^{-1}\hat{\mathbf{S}}_{ab}\mathbf{N}_b^{-1}\hat{\mathbf{S}}_{ba}\bigg]\bigg)^{-1/2}
%\end{equation}
% cosmic variance discussion, still want to check this explicitly

It is important to notice that, even for a PTA with infinite resolution, cosmic variance, polarization of the GW emission, and contributions from the pulsar term will induce deviations from the expected cross-correlations in Eq.~\eqref{eq:theo_corr_disc} (see, for example, Ref.~\ref{}). However, these deviations are well below the current precision at which we are able to reconstruct the cross-correlations (see App.~\ref{} for more details). Therefore, in this analysis, we ignore all these effects. However, as the number of pulsars in PTA data sets increases, and the precision at which we are able to reconstruct cross-correlations improves, taking into account these effects might become necessary. 

%\subsection{Maximum Likelihood sky maps}\label{subsec:rec_maps}


%We choose different resolutions for the recovered sky maps, $N_\text{side}=1,2,4$, and modify the OR matrix in Eq.~\ref{eq:or_matrix} accordingly.\\
%We consider three different approaches for estimating the underlying sky maps from the correlations.\\
%\subsubsection{Radiometer pixel basis}
%The radiometer pixel basis is commonly used to map GW point sources~\cite{Ballmer_2006, Mitra_2008}.
%In the Radiometer pixel basis the Fisher matrix $\mathbf{M}$ is replaced by its diagonal version in Eq.~\ref{eq:ML_solution}. Therefore, all pixels of the sky map are modeled independently, neglecting possible correlations between neighbouring pixels. This approach is only suited for sky maps that contain a single, very bright hotspot~\cite{Romano_2017}. As this is not the case for the majority of realistic SMBHB populations, we do not expect this to be the best approach for our pipeline.
%\subsubsection{Correlated pixel basis}
%Since the radiometer pixel basis is not suitable to recover most of our sky maps, we focus on an exact solution to Eq.~\refeq{eq:ML_solution} by taking  the inverse of the full Fisher matrix and thus including correlations between pixels. This limits the resolution of our maximum likelihood sky maps. For a PTA the general upper limit on the resolution of such a map is given by $N_\text{pix}\leq N_\text{cc}$ \cite{Romano_2017}, which translates to $N_\text{side,max}=8$ for the NANOGrav 15yr configuration with $N_\text{cc}=2211$. We find the inverse of the Fisher matrix to be numerically ill-defined for $N_\text{side}=8$, so that we limit our analysis to $N_\text{side}\leq4$.
%Examples for reconstructed sky maps are given in Fig.~\ref{fig:mock_sky}
%\subsubsection{Numerical Solution}
%In addition to deriving the analytical solution of the maximum likelihood sky map by inverting the full Fisher matrix, we also apply a numerical approach. This allows us to impose positivity on the recovered sky maps and therefore interpret each pixel value as physical power. This approach does not rely on our ability to calculate the inverse of $\mathbf{M}$. Instead, we obtain numerical solutions to
%\begin{equation}\label{eq:num_solution}
%    \mathbf{M}\mathbf{\hat{P}} = \mathbf{X}.
%\end{equation}
%\AL{Should I mention scipy \& the exact function we used here?}

